A Quantitative Analysis of Activities of Daily Living: Insights into Improving Functional Independence with Assistive Robotics

Human assistive robotics have the potential to help the elderly and individuals living with disabilities with their Activities of Daily Living (ADL). Robotics researchers focus on assistive tasks from the perspective of various control schemes and motion types. Health research on the other hand focuses on clinical assessment and rehabilitation, arguably leaving important differences between the two domains. In particular, little is known quantitatively on which ADLs are typically carried out in a persons everyday environment - at home, work, etc. Understanding what activities are frequently carried out during the day can help guide the development and prioritization of robotic technology for in-home assistive robotic deployment. This study targets several lifelogging databases, where we compute (i) ADL task frequency from long-term low sampling frequency video and Internet of Things (IoT) sensor data, and (ii) short term arm and hand movement data from 30 fps video data of domestic tasks. Robotics and health care communities have differing terms and taxonomies for representing tasks and motions. In this work, we derive and discuss a robotics-relevant taxonomy from quantitative ADL task and motion data in attempt to ameliorate taxonomic differences between the two communities. Our quantitative results provide direction for the development of better assistive robots to support the true demands of the healthcare community.

==> Text/abstract.tex <==
... 





\begin{comment}
This paper describes the ...


For some applications, imposing a virtual nonholonomic constraint (VNHC) on the motion of the end effector can help prevent operators from moving in an unintended direction by reducing
the number of controllable degrees of freedom. This paper presents the development of a VNHC for a planar time-delayed telerobotic task, motivated by an on-orbit telerobotic satellite



We also describe a nonholonomic virtual  fixture (NHVF) that adheres to the VNHC to further reduce the potential for operators to input mistaken commands.




servicing operation. We also

This paper introduces a manipulator robot surface
following algorithm using a 3D model of vehicle body panels
acquired by a network of rapid but low resolution RGB-D
sensors. The main objective of this work is to scan and
dynamically explore regions of interest over an automotive
vehicle body under visual guidance by closely following the
surface curves and maintaining close proximity to the object.
The work is motivated by applications in automated vehicles
inspection and screening in security applications. The proposed
path planning strategy is developed based on a perception modeling-planning-action
approach. Raw data rapidly
captured by a calibrated network of Kinect sensors are
processed to provide the required 3D surface shape of objects,
normal measurements, orientation estimation, and obstacle
detection. A robust motion planning method is designed that
relies on this information, resulting in a safe trajectory that is
planned to follow and explore the curved surfaces while
avoiding collision with protruding components of the vehicle.
The feasibility and effectiveness of the proposed method is
validated through experimental results with a 7-DOF
manipulator navigating over automotive body panels. 


he limited bandwidth of sensor-based feedback control restricts the execution speed of a force controlled planar contour following task, if the shape of the workpiece is unknown. This paper shows how appropriate feedforward control of the task frame orientation, calculated online from an eye-in-hand camera image, results in a higher quality (i.e. faster and/or more accurate) task execution. However, keeping the contour in the camera held of view in addition to maintaining a force controlled contact, imposes additional requirements on the controller. This double control problem is specified in the task frame formalism and executed in a hybrid position/force control environment. It is solved using the redundancy for the rotation in the plane, which exists for rotational symmetric tools. The key in this solution is (continuously) redefining the relation between the task frame and the end effector. Experimental results are presented to validate the approach.

In direct teleoperation, 
the users performance was better in bilateral configuration than
the unilateral configuration. In contrast,  our system
both bilateral and unilateral configuration obtain similar
performance, in terms of execution time of task, smoothness of path, 

\end{comment}



==> Text/adl.tex <==



The experiments consist of two main tasks: drawing on a surface and a circular alignment. Users are required to maintain the contact with the surface during the tasks. We conducted a pilot study with 9 users (2 female and 7 male). \kkk The tests were approved by University of Alberta Research Ethics and Managements (Pro00054665). \kkk
All of the users have normal or corrected to normal vision. 
The complete experiment took about 90 minutes per participant. For each task users utilize all 4 different system configurations described in section~\ref{sec:system_description}.  
The sequence of the tasks and the teleoperation configuration was randomized across participants.
At the end of the experiment the users were asked to fill a 21 scale NASA TLX form.

\begin{figure}[h]
\centering
%\includegraphics[trim=2mm 2mm 2mm 2mm, clip=true,width=.48\textwidth] {figures/experimental_setup.eps}
\caption{Three different experiments were conducted using both direct teleoperation and our VF controller. From left to right: line drawing, path drawing and circular alignment tasks.}
\label{fig:experimental_setup}
\end{figure}

\kkk
\subsection{Controller Parameters}
The following controller gains are chosen for all the interface experiments. A nominal force of $F_0 = 4 \, N$ is applied for maintaining the contact. 
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{|l| c c | } \hline
    & Stiffness Gain & Damping Gain \\ \hline
Path Controller & 1000 & 10  \\ \hline
Normal Force Controller & 10 & 0.1 \\ \hline
Tangential Force Controller & 15 & 0.01 \\ \hline
Orientation Controller & diag(7,7,0) & 0.01*diag(1,1,1) \\ \hline
\multirow{2}{*}{Bilateral Controller} & diag(900, 2500,  600, & diag(10,20,5,2, \\
& 500,   50,   50,8) &   0.5,0.5,0.05)  \\ \hline
\end{tabular}
\end{center}
\caption{Controller gains}
\label{table_Controllers}
\end{table}
\subsection{Tasks Description}
\subsubsection{Drawing Task}
The participant is presented with two drawing patterns: a \textit{Line} (Fig.~\ref{fig:experimental_setup}A) and a sinusoidal \textit{Path} (Fig.~\ref{fig:experimental_setup}B). The drawing task consists of tele-operating the remote robot with a pen attached to its end-effector. Users have to make contact with the surface on one end of the pattern and follow it through without lifting the pen from the surface. To perform these tasks users first click on the image to define the desired path. Once defined, users manually activate the VFs  to constrain the robot to the path they defined.

\subsubsection{Circular Alignment Task}
A pattern with two arrows (green and red) is placed on top of a turntable as shown in Fig.~\ref{fig:experimental_setup}C. Initially, the red arrow is aligned with an orange marker. The task is then to align the green arrow with the marked location by rotating the turntable. To rotate the turntable, users have to make contact with the turntable first, and then maintain the contact while rotating in a counter-clockwise circular motion.
%\kkk Again for using the visual interface, user has to click on the image to define the desired (circular) path and then activate the constraints. \kkk  

\kkk
\subsubsection{3D-writing on a Ball}
We demonstrate the capability of our proposed control architecture on a challenging task of following an arbitrary 3D path on a ball. Snapshots of the task are shown in Fig. \ref{fig:3D-task}. Demonstrations of these tasks can be seen in the attached video.   
\kkk
% \begin{figure}[h]
% \centering
% \subfigure[]
% {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.22\textwidth] {figures/ball1.eps}} 
% \subfigure[]
% {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.22\textwidth] {figures/ball2.eps}} 
% \subfigure[]
% {\includegraphics[trim=60mm  5mm 1mm 9mm, clip=true, width=.22\textwidth] {figures/ball5.eps}}  
% \subfigure[]
% {\includegraphics[trim=60mm 45mm 1mm 10mm, clip=true, width=.22\textwidth] {figures/ball7.eps}} 
% \subfigure[]
% {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.22\textwidth] {figures/ball3.eps}} 
% \subfigure[]
% % {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.22\textwidth] {figures/ball4.eps}}
% {\includegraphics[trim=85mm 7mm 85mm 10mm, clip=true, width=.22\textwidth] {figures/3D_sine_path.eps}}
% \caption{Snapshots of tele-operation during the 3D task: [a],[b] user defines the 3D path by clicking in the 2D image interface, [c] Point-cloud visualization of the desired path and the associated normals. [d], [e] user tele-operates the robot using the game-pad, while the proposed VF controller maintains the contact with the 3D surface and reorients the tool. [f] illustration of the end-effector trajectory vs. the defined path.}
% \label{fig:3D-task}
% \end{figure}


% \begin{figure}[h]
% \centering
% {\includegraphics[trim=85mm 7mm 85mm 10mm, clip=true, width=.4\textwidth] {figures/3D_sine_path.eps} }
% \caption{Robot trajectory for the 3D paths on the sphere.}
% \label{fig:Traj-3D}
% \end{figure}

\subsection{Anecdotal Examples}

To proof the applicability of our interface to real world scenarios we complete two anecdotal examples: 1) Closing a steam vale. 2)  Gluing a T PVC pipe.

\subsubsection{Closing a steam valve}
As a proof of concept we run a test during a robot demonstration in an Industrial Mixer at the University of Alberta Computing
Science building. The task consists of closing a steam valve (see Fig.~\ref{fig:steam}) through teleoperating a 7-DOF robot located in the department's 2nd floor, 
with a 4-DOF WAM arm located in our robotics lab (department's 3rd floor). Through this task we show
the viability of using our system in a real task. We noticed that by planing the robot trajectory beforehand the task is carefully laid out and 
obstacles that were hit during direct teleoperation were avoided during the task specification 
(see the video attached).


% \begin{figure}[h]
% \centering
% \includegraphics[width=.45\textwidth] {figures/steam_setup.eps}
% \caption{Anecdotal example during Industrial Mixer at the University of Alberta}
% \label{fig:steam}
% \end{figure}

\subsubsection{Gluing a T PVC pipe}

Our interface allows to specify different magnitudes of normal contact force to complete tasks like welding, polishing, painting, etc. which require moving through a specific path while making contact with a surface. In this example the objective is to apply glue to a crack on a PVC pipe, see Fig.~\ref{fig:tube_task}. 
% During our tests we notice a drift of approximately 1$^{cm}$ to 2$^{cm}$ between the real path to the one followed by the robot. This is due to the Kinect depth error (from a few millimetres up to about 4 cm at the maximum range of the sensor) and  calibration issues between the Kinect sensor and the robot. 

% \begin{figure}[h]
% \centering
% \includegraphics[trim=0mm 0mm 0mm 0mm, clip=true, width=.4\textwidth] {figures/tube_task.eps}
% \caption{Gluing a T PVC pipe: A) The user defines a path on top of the black crack. B) Once the constraints are activated, the user can apply glue by moving the end-effector through the crack. C) The scene point cloud is visualized with the selected path (green spheres) and the calculated normals (green arrows).}
% \label{fig:tube_task}
% \end{figure}





% \begin{figure*}[bht]
% \centering
% \subfigure[\textit{Line}]
% {\includegraphics[trim=23mm 0mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/line_shida_2.eps}} \hfill %line_Tristen.eps
% \subfigure[\textit{Path}]
% {\includegraphics[trim=23mm 0mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/Sine_Kris_2.eps}} \hfill
% \subfigure[\textit{Circle Alignment task}]
% {\includegraphics[trim=23mm 0mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/circle_Tristen_2.eps}}
% \caption{Sample data of a participant performing the three different tasks with the 4 different teleop configurations (uni/bi lateral teleop with/without VF).  The dashed-line is the ground truth path. 
% % and the dotted-line is the path extracted from the interface.  Note that there is a drift between the ground truth and the interface path due to calibration error and user clicking error. %Solid lines colored with green, blue, black, yellow and red represents the trajectories from \textit{uni, bi, uni-VF-C, uni-VF-T} and \textit{bi-VF} teleop configurations, respectively.\kkk
% }
% \label{fig:traj-interfaces}
% \end{figure*}

% \clearpage

\subsection{Results and Analysis}
While performing the task, the position and orientation of the remote robot was recorded for analysis. In addition, when using the interface  the points clicked by the user (hereafter referred to as \textit{interface path}) are recorded. 
Trajectories of the end-effector controlled by one of the participants are shown in Fig.~\ref{fig:traj-interfaces} for different tasks and with different teleop configurations. \kkk The red dashed-line represents the  ground truth path, which is obtained by moving the tip of the robot to the desired path and recording the pose. \kkk 
% the and black dotted line represents the desired path from the interface. 
% We attribute the offset between these two lines to three main factors: (1) The accuracy of the Kinect sensor used, (2) Kinect-robot calibration error, and (3) user input error.
It is clear from Fig.~\ref{fig:traj-interfaces} that each teleop configuration presents a different characteristic behaviour in the tasks.
The following four metrics are used to characterize/evaluate the performance of teleop configurations.

\subsubsection{Path Smoothness}
The smoothness of each path was assessed using the \textit{Spectral Arc Length} (SAL) metric developed in \cite{smoothness_measure}. SAL is a dimensionless measure of the length of the frequency spectrum curve of a 
speed profile over the bandwidth appropriate for the motion. 
For a movement with speed profile $v(t)$, SAL is calculated from
$$SAL := \int_0^{\omega_c} \sqrt{ \big({\tfrac{1}{\omega_c}}\big)^2 + \big( { \tfrac{dV(\omega)}{d\omega} } \big)^2 } d\omega.$$
where $V(\omega)$ is the Fourier magnitude spectrum of $v(t)$, and
$[0,\omega_c ]$ is the frequency band spanned by the given movement. 
$\omega_c = 40 \pi$ rad/s (which corresponds to 20 Hz) covers the normal
and abnormal aspects of human movements \cite{smoothness_measure}. 
It should be noted that SAL value approaches zero with increases in smoothness of the path. 
% \begin{figure}[h]
% \centering
% \subfigure
% {\includegraphics[trim=6mm 6mm 1mm 7mm, clip=true, width=.4\textwidth] {figures/smoothness.eps} }
% \subfigure
% {\includegraphics[trim=5mm 5mm 1mm 7mm, clip=true, width=.4\textwidth] {figures/execution_time.eps} }
% \caption{Comparison of (top) the smoothness of the paths, (bottom) execution time of the tasks for different teleop configurations.}
% \label{fig:smoothness_compare}
% \end{figure}

Figure \ref{fig:smoothness_compare} (top) compares the smoothness of the paths for different teleop configurations and for different tasks. It can be seen from this figure that  VF improves the smoothness of the paths. \kkk As expected, game-pad teleop configuration results in the most jerky (non-smooth) motions. Adding the virtual fixtures significantly improves the smoothness of the paths.  In fact, the smoothness of the paths with uni-VF configuration is (on the average) better than bilateral configuration and comparable with bilateral with VF configuration. This is due the fact that in uni-VF mode, the operator is only able to move the robot along the path. \kkk


\subsubsection{Time to complete the task}
Figure \ref{fig:smoothness_compare} (bottom) compares the execution time of each task for different teleop configurations. 
Note that the time to set the path from the interface is not considered here in the measurements as this procedure can be done offline.
It can be seen from this figure that VF reduces the execution time of  the tasks in unilateral configuration.  \kkk Uni-VF performed the best as anticipated; adding a driving force in the tangential direction helps the operator to finish the task faster. \kkk


% \begin{figure}[h]
% \centering
% \includegraphics[trim=10mm 1mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/execution_time.eps}
% \caption{Execution time of the tasks for different teleop configurations.}
% \label{fig:time_compare}
% \end{figure}

\subsubsection{Trajectory Error}

% As expected uni-VF paths are all close to the interface path instead of the ground truth. This is due to the fact that the constraints are generated from the interface path. For the bi-VF, we noticed users attempting to compensate for the calibration and input errors as they directly observe the robot and the ground truth.
Table \ref{table1} presents the trajectory mean error (averaged over all participants) for the line and sinusoidal paths. \kkk Given the ground truth path ($\bm P_{GT}$), the  error from the path is computed as the minimum distance of the sampled trajectory to the path, \textit{i.e.} 
$ e( \bm x)  = \min_{\bm p \in \bm P_{GT} } \| \bm x - \bm p \|$. \kkk
% Two errors are reported. The first one, $e_{GT}$, is the difference between the trajectory and the Ground Truth (blue dashed-line in Fig. \ref{fig:VFT_results}).
% The second error, $e_{IP}$, is computed as the difference between the trajectory and the interface path (black dotted-line in Fig. \ref{fig:VFT_results}).  
% $e_{GT}$ is used for the uni, bi, and bi-VF configurations because the operator directly see the ground truth. 
%The drift between the ground truth and the generated path from the visual interface is mainly due to the inherent error of the RGB-D sensor and also error in the sensor-to-robot calibration.  
% In order to take into account the calibration error, we use $e_{IP}$ for the teleop configurations with visual-force assistance as the measure of trajectory error. 
\kkk It can be seen from Table \ref{table1} that the bi-VF has the best performance in terms of trajectory following. While the performance of the unilateral teleop is not satisfactory,  adding the VF significantly improve the performance of the uni-VF teleop up to a point that is comparable to bi-VF. Note that the error in the bilateral configuration is higher compared to  uni-VF control. 
This observation is in line with the one of \cite{castillocruces2009},  
because in  bilateral mode, operator has to control both position and orientation simultaneously. 
Authors of \cite{castillocruces2009} stated that this is due to the translational and rotational components of motion being decoupled from each other in such a way that the user, focusing on moving one, will not notice an error in the other and vice versa.  
The same trend is observed in the variance of the errors, except that the variance of the error is smaller for the uni-VF. This could be due the fact that in the uni-VF mode, the operator is only able to move along the path direction. In the bi-VF mode, however the operator is able to fight with VF and move in other directions. 
\kkk
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{|lr|c c c c | } \hline
%\multicolumn{2}{c}{Example 1  }  \\ \hline
\multicolumn{2}{|c|}{}                    & uni & bi  & uni-VF  & bi-VF \\ \hline
\multirow{2}{*}{Line} & mean error (mm)  & 13.78  & 11.76  & 4.50 & \textbf{4.37}    \\ 
    & variance (mm)  & 8.15 &	5.96  &	\textbf{1.52} &	2.19     \\ \hline
\multirow{2}{*}{Path} & mean error (mm)  &  13.99    & 11.13  & 9.08 & \textbf{8.51}    \\ 
    & variance (mm) & 9.58    &	7.53  &	\textbf{4.07} &	3.42    \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of the trajectory error and variance for different teleop configurations}
\label{table1}
\end{table}

\subsubsection{Loss of Contact}
Table  \ref{table2}  compares the average number of times that the robot's end-effector tip lose the contact with the surface during the experiments. In the simple uni-lateral control, it is hard for the operator to maintain the contact with the environment due to the lack of haptic feedback through the game-pad.  Contact control improves in the bilateral case as the user is able to feel the force feedback from the remote site and tries to maintain the contact. Table \ref{table2} shows the effectiveness of the normal force controller in maintaining the contact with the environment. 
% \begin{figure}[h]
% \centering
% \includegraphics[trim=23mm 2mm 1mm 7mm, clip=true, width=.3\textwidth]
% {figures/all_lines_VF_2.eps}
% \caption{Paths traced by different users with uni-VF and bi-VF teleop configurations}
% \label{fig:VFT_results}
% \end{figure}
% Figure \ref{fig:VFT_results} shows the path traced by four participants using both uni-VF and bi-VF teleop configurations. 
\kkk
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{|l|c c c c | } \hline
        & uni & bi  & uni-VF  & bi-VF \\ \hline
Line    & 2.71  & 0.75 & 0 & 0        \\ \hline
Path    & 3.33  & 1.14 & 0.28 & 0     \\ \hline
\end{tabular}
\end{center}
\caption{Average number of loss of contact with the surface during the line /path following tasks}
\label{table2}
\end{table}
\kkk

In summary, the the performance of the unilateral with VF in terms of error, execution time, smoothness of the path and contact control is comparable to the one of bilateral control with VF. This also signifies that lack of haptic feedback in the unilateral control can be compensated by proper integration of vision and force control.

\subsubsection{Operator Workload Measure}
Figure \ref{fig:TLX} shows the mean ratings of each workload category reported by the users in the NASA TLX survey. 
The uni-VF configuration resulted in less overall workload than all the other configurations including the bi-VF. This again confirms our hypothesis that by
introducing  vision-force assistive constraints, the operator's performance in the unilateral case can be improved, perhaps up to the point where performance is similar to the bilateral configuration.
\begin{figure}[h]
\centering
\includegraphics[width=.4\textwidth] {figures/NASA_TLX.eps}
\caption{Nasa TLX radar plot: Qualitative workload evaluation, higher workloads are farther from the center of plot.}
\label{fig:TLX}
\end{figure}








\begin{comment}

% \begin{figure}[h]
% \centering
% \includegraphics[trim = 5mm 0mm 5mm 5mm, clip=true,width=.3\textwidth] {figures/paths.eps}
% \caption{Paths: a) linear (2D), b) circular (2D), c) path between way-points, d) path on a 3D surface.}
% \label{fig:paths}
% \end{figure}



\kkk 3D task \kkk

A- tele-op with joystick



B- tele-op with haptic feedback

-- ) only tele-op without assistive visual/force fixtures

-- ) tele-op with assistive visual/force fixtures 


\rrr 
 the metrics are : -1 smoothness of the path , 2) the time to complete the task, 3) the error, 

 experiment variables: 1) remote device ( joy-stick = non-symmetric config. , wam - wam = sym. config.) 
                        2) delay
                        3) force / no-force ( contact  force feedback) 
                        4) Visual Fixture / No VF (with only visual feedback ) 
                        5) user velocity

                        
=> the conclusion : hypothesis is that non-sym tele-op with assistive VF will have the similar performance of the sym configuration with visual/force assist 
while non-sym tele-op is worse than the sym teleop  without the VF.
\kkk 


\rrr 
Future work: 
Consider the effect of friction, model of the friction force to compensate for it.  

\kkk



\begin{figure}[h]
\centering
\includegraphics[trim=23mm 0mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/line_VFT_biVF_compare.eps}
\caption{Comparison of line following with uni-VF-T interfaces and bi-VF}
\label{fig:VFT_results}
\end{figure}


\end{comment}














==> Text/conclusions.tex <==
We present the design and implementation of a novel flexible virtual fixture interface.
%We present the design and implementation of a new interface for flexible force-vision-based system.
By allowing users to visually specify path constraints for a tele-manipulation task we were able to provide a system where performance of unilateral (gamepad - WAM) configurations began to match that of a bilateral (WAM - WAM) system. The lack of feedback in unilateral control was compensated through our interface. In our pilot user study  smoothness (SAL metric) was improved by a factor of 2 over all the tasks performed by users when using our interface. Similarly users were able to reduce the task time by a factor of 2.1. Reducing the  control degrees of freedom,  results in reducing their perceived workload. The users not only prefer  to use our teleop interface, but their performance is also improved. One area of future work is the study of the effects of calibration error on our system. When users try to fight the forces introduced by the system, we see a serious increase in the trajectory error. User's attention is more focused  on trying to correct for the calibration offset rather than on completing the task which  results in performance degradation and  increase in mental demand.

==> Text/introduction.tex <==
Tele-robotics has brought humans the capacity of changing the physical world remotely. This has made a big impact on many fields. Some examples are: Surgery, disaster response robotics, under-water and space exploration. Recently DARPA conducted the robotics challenge where robots controlled through semi-autonomous teleoperation  completed tasks hazardous to humans.
 %Exploration in under-water environments, or in space, are two more examples.  It has also been shown to have a significant potential in disaster response robotics, as shown in the DARPA challenge.
Yanco \etal~\cite{yanco2015analysis} study the different group performances during the challenge.  They concluded that the use of effective semi-autonomous routines, in combination with sensor fusion, and an easy to use interfaces for users lead better performance. % Therefore providing a well elaborate interface is a requirement for a good task performance. 
Perhaps the most desirable capabilities to fuse during robot manipulation are vision and force.
Common vision-force control approaches use impedance-based and hybrid-based strategies~\cite{mezouar2007external}. In the former a vision based controller drives the movement of the robot's end-effector and the force controller provides compliance to external disturbances~\cite{morel1998impedance}. While, in the latter, vision and force controllers are working in parallel  and thus it is necessary to ensure orthogonality between both controllers to avoid any conflict at the actuator level \cite{hosoda1996adaptive, pichler2000uncalibrated}.  The main role of vision-force control in tele-manipulation is to assist the operator by  generating motion guidance active constraints  also known as \textit{Virtual Fixtures} (VF).

These constraints are typically used to either restrict the movement of the robot to certain regions (forbidden region VF) or to  guide the operator through a specific path (guidance VF)~\cite{bowyer2014active,Okamura_2004}. VFs reduce the  task complexity and operator's workload. They have been  used  in many applications, for example polishing/finishing mechanical  parts~\cite{nee2014handbook}, automotive inspection~\cite{TrajectoryPlanningSurfaceFollowing}, robot-assistive surgery~\cite{okamura2004methods,PointCloud_VF_2013,DynamicVF_2007}, human-robot cooperative tasks \cite{castillocruces2009} or space exploration~\cite{VF_ICRA_2015,VF_IROS_2012,VF_ICRA_2013}. 




\begin{figure}[t]
\centering
%\includegraphics[width=.48\textwidth] {figures/system_and_example.eps}
\caption{The use of our proposed interface is illustrated by closing a steam valve in a remote location. I) The local operator is provided with a monitor displaying our interface and a game-pad for interaction. II) In the remote site a 7-DOF WAM arm is teleoperated with the aid of our interface to close a steam valve. \textbf{A} and \textbf{B} show the RGB and Point Cloud visualization of our interface. 
% \textbf{A}, \textbf{B}, \textbf{C} and \textbf{D} shows the use of the interface by the operator to close the valve. 
A) The operator defines a desired path in the 2D image by clicking (blue dots). B) The 3D path and the associated normals to the surface are calculated and visualized (green spheres and green arrows). C, D) Once the constraints are activated the user can complete the task by simply controlling 2-DOF: motion through the path direction and motion normal to the surface.  
}
\label{fig:teleop_setup}
\end{figure}




%\begin{figure}[t]
%\centering
%\includegraphics[trim=1mm 5mm 1mm 1mm, clip=true, width=.48\textwidth] {figures/remote_drawing.eps}
%\caption{Left: A local operator specifies through our visual interface a path to draw an arch. Right: Both local and remote robots are constrained to path $\bm p$. Forces $F_n$ and $F_t$ are applied to keep the contact with the surface and to assist motion along the path, respectively.
% Notice that in this particular case, the path is defined on a planar surface. However our system is capable of defining a path on any 3D surface 
% (see e.g. Fig. \ref{fig:visual_interface}).
%}
%\label{fig:teleop_setup}
%\end{figure}

One of the biggest challenges in applying VFs in real world tele-robotics scenarios is to find a way to provide flexible and efficient geometric constraints specification~\cite{bowyer2014active}.  
% \rrr As pointed out by ~\cite{bowyer2014active} currently one of the biggest challenges in the use of VFs in tele-robotics, is to efficiently specify the geometric  constraints.

For example, authors of \cite{Flexible_VF_2013} propose a flexible VF that can be adjusted in  the presence of an obstacle in the path. In \cite{castillocruces2009}, an autonomous error compensation method is presented to overcome human difficulties in simultaneously controlling the position and orientation of a 6-DOF robot under reference direction fixtures \cite{castillocruces2009}. Authors of \cite{castillocruces2009} proposed a dynamic VF for robot-assisted surgery. While there are several attempts, geometric constrain specification is still a challenging problem \cite{bowyer2014active}.
We address this problem through the design of a novel 2D interface that allows the operator to intuitively generate a 3D VF for the remote manipulator on top of the image stream coming from the remote location. Furthermore, we present the design of \kkk a tele-manipulation system that aims to improve an operator's performance and reduce his/her workload independently of the master device. \kkk Our main contributions are:
\begin{itemize}
    \item A 2D image interface that simplifies the complex process of specifying a 3D path constraint to a remote manipulator.
    \item \kkk An impedance control architecture that constrains the robot manipulator to follow a 3D path, while maintaining the contact with the environment. The controller is specifically appealing for tasks that require contacts with the \kkk environment. 
    \item Integration of an image interface and VF control architecture that provides a flexible system permitting both bilateral and unilateral teleoperation with or without path constraints.
    \item Quantitative and qualitative evaluation of our system through a 9-participant user study, that compares the unilateral and bilateral configurations with and without the path constraints.
    % \item Two different implementations of unilateral control. One through a Cartesian force controller and the second one through forces applied along the user defined path and its normal direction.
    % \item A case study showing the potential of our designed system solving a 3D task.
\end{itemize}
The rest of this paper is organized as follows: section \ref{sec:system_description} outlines the problem formulation and the overall system description and development.  Section \ref{sec:experiments} describes the experimental setup, procedure, results and discussion on findings. Conclusions and future works are presented in section \ref{sec:conclusions}.


%Section \ref{sec:experiments} describes the setup and the procedure used for the user tests and presents the experimental results and discussion on the findings. 
% Then Section \ref{sec:case_study} present a case study to illustrate how our system can be used on achieving a 3D task. 



% \begin{figure}[h]
% \centering
% \includegraphics[trim=1mm 5mm 1mm 1mm, clip=true, width=.48\textwidth] {figures/remote_drawing.eps}
% \caption{Left: A local operator specifies through our visual interface a path to draw an arch. Right: Both the local and remote robot are constrain to path $\mathbf p$. A force $F_n$ and $F_t$ are applied to keep contact to the surface and to assist during the path movement, respectively. Notice that in this particular case, the path is defined on a flat surface. However our system permits definition on top of any 3D surface.}
% \label{fig:teleop_setup}
% \end{figure}




\begin{comment}



A practical application using a hybrid position-force control and active constrains to complete a space related task is presented by  Leonard \etal \cite{VF_ICRA_2013, VF_ICRA_2015}. The task consists on using a master interface (da Vinci Research kit) to control a remote slave robot (7DOF WAM arm) to cut a tape that secures a flap of multi-layer insulation over the access panel of a satellite  mockup. They show experimentally that force control based on a virtual fixture can increase operator performance an decrease workload. 








Vozar et al. ~\cite{VF_IROS_2015} present the development of a virtual nonholonomic constrain to achieve a planar telerobotic task.  They showed experimentally through a pilot study that their approach has comparable task performance to a holonomic planar teleoperation, while decreasing operator load.  Later in ~\cite{VF_ICRA_2015} force control in the axis normal to the plane was observed to improve task quality and reduced operator workload by regulating an additional component of the end effector’s position.


Similar to cutting writing also requires a constant force applied normal to the trajectory path to keep the marker/pen in contact with the drawing surface.
Similar to Yanco, we believe that by the correct use of sensor fusion and providing well defined semi-autonomous tools to the human operator, the performance and task success rate will increase.
Different control architectures have been proposed to combine force and vision 

-- Intro ... - motivation --  why extraction surface normal + visual fixture is important 

Hybrid force/vision 


Applications of on a 3D surface include, polishing/finishing of a marine propeller \cite{}, seal the gaps, taping  
welding 

Vozar et al. ~\cite{VF_IROS_2015} present the development of a virtual nonholonomic constrain (VNHC) to achieve a planar telerobotic task. 
They showed experimentally through a pilot study that the VNHC has comparable task performance to a holonomic planar
teleoperation, while decreasing operator load.  

In ~\cite{VF_ICRA_2015} force control in the axis normal to the plane was observed to improve task quality and reduced operator workload by regulating an additional component of the end effector’s
position.







\kkk
that presently it is virtually impossible to perform complex manipulation tasks with robotic
manipulators in unstructured environments. While the highly
structured known environment of the assembly line has
enabled successful robotic automation of structured manipulation tasks in manufacturing, robotics has had comparatively
little impact in less structured manipulation tasks such as
surgery and machine assembly/disassembly/repair due to
the uncertainty arising in these tasks and environments.


By combining human strengths in reasoning and high-level
strategy with machine capabilities in information fusion,
task planning, and simulation, we can manage uncertainty
and achieve successful human-robot partnerships to perform
complex tasks in uncertain environments that were previously considered impractical or infeasible.

\kkk



-- Related works ... review of two main Hybrid Vision/Force Control schemes - what is missing - ...

-- Contributions ... + (possible) applications

Most of the works are for 2D virtual fixtures. This work however, presents a 3D visual assistive fixture by defining a path. The path normals are also included.


\kkk

We do not yet consider bandwidth constraints, which may
reduce the quality (resolution) of video feedback unless they
can be overcome by image compression methods or future
improvements to the communication infrastructure.

The key contribution of our work is the development of
an augmented reality framework that enables the operator to
design and implement assistive fixtures when confronted with
an unknown task in an unstructured environment unsuitable
for autonomous systems. Although motivated by our research
in medical robotics (where we extensively use virtual fixtures
and augmented reality overlays), this framework represents
a new development in either domain.

\kkk 



\cite{HybridVisionForce} 
\cite{FingerContactSensing,PredictiveContourFollowing,TrajectoryPlanningSurfaceFollowing,ContourFollowing,AdaptiveVisionForce,IntegratedVisionForce,MultiSensorContourFollowing,DoorOpening}

\cite{VF_parameters_IROS_2015}
\cite{VF_IROS_2012}
\cite{VF_ICRA_2013,VF_ICRA_2015,VF_IROS_2015,VF_parameters_IROS_2015}
\cite{rusu2013semantic}
\cite{rusu20113d}
\cite{holz2011real}
\cite{holzer2012adaptive}
\cite{bowyer2014active}
\cite{yanco2015analysis}

\cite{pratt2013darpa}

\end{comment}




==> Text/related_works.tex <==
The general task that we are addressing is to tele-operate a robot manipulator while guiding it through a desired path (see Fig. \ref{fig:teleop_setup}).
In these applications, direct bilateral teleoperation is often preferred as it results in better operator's performance when compared to unilateral control.

Our hypothesis, however,  is that by introducing a vision-assisted control system which is capable of generating VFs, 
% and provide an intuitive way to specify constrains
the operator's performance in the unilateral case can be improved, perhaps up to a point where performance is similar to the bilateral configuration.



\begin{figure}[h]
\centering
% \includegraphics[width=.4\textwidth] {figures/modes.eps}
\caption{Different teleoperation configurations. 1) \bf{uni}:gamepad to WAM 7-DOF; in this configuration there is not force feedback. 2) \bf{bi}: 4-WAM with 3-DOF gimbal to WAM 7-DOF; in this configuration there is force feedback. 3) \bf{uni-VF}: uni configuration with aid of the interface. 4) \bf{bi-VF}:bi configuration with aid of the interface.}
\label{fig:modes}
\end{figure}

In order to test our hypothesis, we
have implemented different teleoperation configurations, see Fig.~\ref{fig:modes} :
\begin{itemize}
    \item Direct Unilateral (\textit{uni}): This is a unilateral configuration where the local operator controls the remote robot through a game-pad. A Cartesian force controller is actuated through a game-pad to control the remote robot. 
    \item Direct Bilateral  (\textit{bi}):   Both local and remote robots are linked. This configuration allows the local operator to control each joint of the remote robot by physically manipulating the corresponding joint of the local one. We use a similar approach to the one proposed by Glover \etal~\cite{glover2009effective} to provide  haptic feedback to the local operator from the remote robot. 
   % \rrr In our setup, a 4-DOF robot arm is used as the local side and a 7-DOF in the remote side. The system reorients the last 3-DOF of the remote robot towards the normal direction of the surface obtained through the visual module (Section \ref{subsec:visual_module}). \kkk
  	\item Unilateral with Virtual Fixture (\textit{uni-VF}): 
  	Similar to unilateral configuration plus VF constraining the remote robot's end-effector to the specified path. 
  	\item Bilateral with virtual fixture (\textit{bi-VF}): The same linking described in the Bilateral configuration. In addition, the remote robot is constrained to a path specified using our force-vision module.
\end{itemize}

In summary our system implementation provides both unilateral and bilateral teleoperation for a 7-DOF WAM arm. In the unilateral case the remote robot arm is tele-operated with a game-pad, while in the bilateral case a 4-DOF WAM arm with a 3-DOF gimbal is used as the master manipulator. To provide the path following functionality to the 7-DOF WAM arm, our system relies on three modules: \textit{Visual Interface}, \textit{Control} and \textit{Vision} as shown in Fig.~\ref{fig:system_overview}.

\begin{figure}[h]
\centering
%\includegraphics[width=.45\textwidth] {figures/system_overview.eps}
\caption{System overview. Left: The I/O devices that the local operator interacts with, are the mouse, screen, game-pad and 4-DOF WAM arm. The first two are used for monitoring the remote location and for specifying the desired path constraints. Game-pad is used for the unilateral teleoperation and the 4-DOF WAM arm for the bilateral teleoperation. Right: The vision and control module are in-charge of processing the RGB-D sensor information and constraining the 7-DOF WAM arm to the specified path.}
\label{fig:system_overview}
\end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=.45\textwidth] {figures/interface_fig2.eps}
% \caption{test}
% \label{fig:system_overview}
% \end{figure}

\subsection{Visual Interface Module}
\label{subsec:visual_module}

The \textit{Visual Interface} (Fig.~\ref{fig:visual_interface})
 is equipped with a drawing tool that allows the operator to define a desired trajectory on the image stream from the remote site.
The interface also provides a real time point cloud visualization in which the operator can corroborate visually the selected 3D path and the corresponding estimate of the surface normals.


\begin{figure}[h]
\centering
%\includegraphics[trim=0mm 0mm 0mm 0mm, clip=true, width=.30\textwidth] {figures/interface2.eps}
\caption{Visual Interface: A) By clicking on the image the user set a path on top of the surface. B) The scene point cloud is visualized with the selected path (green spheres) and the calculated normals (green arrows).}
\label{fig:visual_interface}
\end{figure}


% \begin{figure}[h]
% \centering
% \subfigure[]
% {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.23\textwidth] {figures/ball1.eps}} 
% \subfigure[]
% {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.23\textwidth] {figures/ball2.eps}} \\
% \subfigure[]
% {\includegraphics[trim=60mm  5mm 1mm 15mm, clip=true, width=.23\textwidth] {figures/ball5.eps}}
% % \subfigure[]
% % {\includegraphics[trim=60mm 45mm 1mm 10mm, clip=true, width=.15\textwidth] {figures/ball7.eps}} 
% % \subfigure[]
% % {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.15\textwidth] {figures/ball3.eps}} 
% % \subfigure[]
% % {\includegraphics[trim=60mm 30mm 1mm 7mm, clip=true, width=.15\textwidth] {figures/ball4.eps}}
% \caption{Visual Interface: \bbb (a),(b) By clicking on the 2D image the user set a path on top of a surface. (c) Visualization of the scene point cloud with the selected path (green spheres) and the calculated normals (green arrows). \kkk}
% \label{fig:visual_interface}
% \end{figure}

\subsection{Vision Module}

The \textit{Vision module} streams the video coming from an RGB-D sensor in the remote location to the visual interface presented to the operator. In our tests we utilize a Kinect sensor. This module feeds the \textit{Control module} with the 3D path coordinates and corresponding surface normals with respect to the robot reference frame. The 3D path coordinates are found using the direct correspondence of the RGB sensor and depth sensor. These are then converted into robot coordinates through a Kinect-Robot transformation matrix (previously calculated using a calibration routine). The typical approach to calculating surface normals consists of fitting a plane to the neighborhood $P_i$ of the target point $p_i$.  $P_i$ is either formed by the $k$ nearest neighbors of $p_i$ or by points within a radius $r$ from $p_i$. Given $P_i$, its covariance matrix $\bm C_i$ ${\in}$ ${\rm I\!R^{3x3}}$ is computed (see ~\cite{rusu2013semantic} for details of the computation).
The eigenvectors of the covariance matrix, ${\bm v}_{i,0}$, corresponding to the smallest eigenvalue $\lambda_{i,0}$, can be used as an estimate of the target normal $\hat {\bm n}_i$~\cite{rusu2013semantic}.     
To reduce the computational time and achieve real time performance, we used the integral normal estimation approach. %implemented in the \textit{Point Cloud Library} (PCL)~\cite{rusu20113d}
This implementation takes advantage of the organized structure of the point cloud acquired by the RGB-D sensor and also uses a pixel neighborhood instead of a spatial neighborhood.
By using the pixel neighborhood the simplest approach is to use the right-left pixels and up-down pixels to form two 
local tangential vectors and calculate the normal using the cross product. However, since the data is noisy due to the
nature of the sensor, an average tangential vector calculation (known as a integral image \cite{holzer2012adaptive}) is performed. 
In our implementation we use the PCL~\cite{rusu20113d} \textit{Average 3D Gradient} mode which creates 6 integral images to compute smoothed versions of horizontal and vertical 3D gradients and computes the normals using the cross-product between these two gradients \cite{holz2011real}.




\subsection{Control Module}
This section describes the details of the controller module for remote robot. Our robot is a torque controlled 7-DOF WAM manipulator with the dynamic equation of
\begin{align*}
\bm {M}(\bm q) \ddot {\bm q} + \bm {C}(\bm q,\dot {\bm q})\dot {\bm q} + \bm g(\bm q) = \bm {\tau} + \bm {\tau}_{ext}
\end{align*}
where $\bm q$ is the joint angles, $\bm {M}(\bm q)$ is the positive-definite inertia matrix, $\bm {C}(\bm q,\dot {\bm q})$ is the Coriolis matrix, ${\bm g}(\bm q)$ is the gravitational force, $\bm {\tau}$ the actuators torques, and $\bm {\tau}_{ext}$ is the external generalized force applied to the robot by the environment.
\begin{figure}[h]
\centering
\includegraphics[trim = 35mm 140mm 60mm 60mm, clip=true, width=.35\textwidth] 
%{figures/force_diagram.eps}
{figures/surface.eps}
\caption{Schematic of the path on a surface and construction of the corresponding path reference frame.}
\label{fig:surface_coordinates}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[trim = 1mm 1mm 1mm 4mm, clip=true,width=.4\textwidth] 
{figures/controller2.eps}
\caption{Control architecture of the remote robot.}
\label{fig:Controller}
\end{figure}
As shown in Fig. \ref{fig:surface_coordinates}, the goal of the controller is to constrain the robot end-effector to the path (on a surface) while maintaining a contact force ($F_n$) on the surface. This is achieved by projecting the motion onto orthogonal directions along the tangential ($\hat {\bm t}$), normal ($\hat {\bm n})$ and side directions ($\hat {\bm s})$, see Fig. \ref{fig:surface_coordinates}. A dedicated controller is then designed for each direction. An additional controller is also required for orienting the robot's tool.  
The proposed control architecture is shown in Fig. \ref{fig:Controller} and it is composed of a \textit{Constraint Evaluation} module and four sub-controllers.
% , namely 1) Path controller, 2) normal force controller, 3) tangential force controller and 4) orientation controller.
\kkk
It is assumed hereafter that the visual interface module provides the desired path, i.e. a collection of 3D points on the surface ($ \{ \bm {x}_{d_i}\} $).
Then, the inputs to the controller are (i) the desired path ($ \{ \bm {x}_{d_i}\} $) and (ii) the corresponding normal directions at each point ($\{ \hat {\bm  n}_i \}$).  Details of each of the modules are given next. \kkk
\subsubsection{Constraint Evaluation}
The initial step to decide on the direction of anisotropy of the active constraint, is to find the relative configuration of the robot and the constraint \cite{bowyer2014active}. Following the methodologies of \cite{Okamura_2004},  the desired point  $\bm {x}_{d_i}$ is the closest point on the reference path to the robot's tool tip $\bm x$. Thus, for any given $\bm x$, the corresponding $\bm x_d$ is obtained from:
\begin{align}
   \bm {x}_{d} (\bm x) := \arg \min_{\hat{\bm x} \in \{ \bm {x}_{d_i}\} } \| \hat{\bm x} - \bm x \|
\label{eqn:min_dist}
\end{align}
\subsubsection{Path controller} 
% The first thing is to find the tangential direction of the path (see Fig. \ref{fig:surface_coordinates}). 
Given the desired path, the tangential direction at each point is computed first by $\hat {\bm t}_i = \bm {x}_{d_i} - \bm {x}_{d_{i-1}}$. From this and the given normal direction, the path reference frame is fully characterized by $ \{ \hat {\bm n}, \hat {\bm s}, \hat {\bm t} \}$, where 
$\hat {\bm s} = \hat {\bm n} \times \hat {\bm t}$ (see  Fig. \ref{fig:surface_coordinates}). Path controller is responsible for forcing the end-effector to be constrained to the path in the $\hat {\bm s}$ direction. To this end, let $ \bm d = \bm x - {\bm x}_d$ be the minimum distance of the end-effector tip to the path from (\ref{eqn:min_dist}). 
An impedance controller is then used to minimize the projection of $\bm d$ onto $\hat {\bm s}$ direction. To this end, define
\begin{align}
F_{s} = K_{p_{p}} \big( (\bm x - \bm x_d) \cdot \bm {\hat s} \big) +  K_{d_{p}} (\bm {\dot x} \cdot \bm {\hat s})
\end{align}
as the magnitude of the side direction force, due to the virtual spring $K_{p_{p}}$ and damper $K_{d_{p}}$ system that pulls $\bm x$ towards point $\bm p$ on the reference path. The torque command that generates this force is  
\begin{align}
\bm \tau_{p} = \bm J^T ( F_s \:  \hat {\bm s} )
\end{align}
where $\bm J$ is the task Jacobian matrix of robot.
\subsubsection{Normal Force controller} This compliance controller is responsible for maintaining the contact with the surface by applying a  normal force ($F_n$) in the  $-\bm{\hat n}$ direction:
\begin{align}
&F_{n} = K_{p_{n}} \big( (\bm x - \bm x_d) \cdot \bm {\hat n} \big) +  K_{d_{n}} (\bm {\dot x} \cdot \bm {\hat n}) + F_0 \\
&\bm \tau_n =  - \bm J^T (F_n \: \bm{\hat n})
\end{align}
where $F_0$ is the nominal desired force to be applied on the surface. 
\subsubsection{Tangential Velocity controller} This controller drives the robot's end-effector in the path direction with a desired tangential velocity $v_d$: 
\begin{align}
&F_{t} = K_{p_{t}}  ( \bm {\dot x} \cdot \bm {\hat t}  - v_d) 
+  K_{d_{t}} (\bm {\ddot x} \cdot   \bm {\hat t} - \dot v_d ) \\
&\bm \tau_t =   \bm J^T (F_t \: \bm{\hat t}).
\end{align}
% $ \bm \tau_t = \bm J^T (F_t \: \bm{\hat t})$.
\subsubsection{Orientation controller} Lastly, an additional controller is needed to align the end-effector to the desired orientation. To this end, the following compliance controller is used
\begin{align}
     \bm \tau_o =  \bm K_{p_o}  (\bm o - \bm o_d) + \bm K_{d_o} (\bm {\dot o}) 
\end{align}
where $\bm o_d, \bm o$ are the desired and actual orientation of the robot's end-effector.
In the general case, the desired orientation $\bm o_d$ is path dependant. Here we assume that the end-effector (tool) reference frame $\{X_t, Y_t, Z_t\}$ is reoriented such that $Z_t$ is aligned with $\text{-} \hat {\bm n}$ and $Y_t$ is aligned with the tangential direction $\hat {\bm t}$. The rotation matrix from tool to base is then $\bm R_t^b = [\hat {\bm s} , \hat {\bm t} ,  \text{-}\hat {\bm n}]$ from which $\bm o_d$ is obtained.





The final
actuator torque command $\bm \tau$ that is sent to the robot is
\begin{align}
   \bm{\tau} = \bm \tau_g +  (\bm \tau_c + \bm \tau_n + \bm \tau_t + \bm \tau_o  ) + \bm \tau_l
\end{align}
where $\bm \tau_g = \bm g(\bm q) $ is the gravity compensation torque and $\bm \tau_l$ is the  torque command received from the local end (either from the game-pad in unilateral configuration or from the WAM in bilateral configuration). 
% Note that once the path has been specified, an initial step is required to find the closest $\bm x_d$ of the path to the current end-effector position $\bm x$. This is done by a simple minimum distance search along the path.
In the  bilateral configuration, \\ $\bm \tau_l = \bm K_{p_l} (\bm q_r - \bm q_l) + \bm K_{d_l} (\bm {\dot q}_r - \bm {\dot q}_l)$.  



\begin{comment}
An integral image IO corresponding to an image O makes
it possible to compute the sum of all values of O within
a certain rectangular region R(ms,ns)->(me,ne)

To perform this averaging integral images
is performed.
It consist in create two maps of tangential vectors, one for the u- and one for the v-direction. 
The vectors for these maps are computed between corresponding 3D points in the point cloud. 
That is, each element of theses vectors is a 3D vector. For each of the channels (Cartesian x, y, and z)
of each of the maps we then compute an integral image, which leads to a total
number of six integral images. Using these integral images, we can compute the
average tangential vectors with only 2 × 4 × 3 memory accesses, independent of
the size of the smoothing area. The overall runtime complexity is linear in the
number of points for which normals are computed     

... 
\end{comment}


% \begin{figure}[h]
% \centering
% \includegraphics[trim = 50mm 175mm 30mm 50mm, clip=true,width=.45\textwidth] {surface.eps}
% \caption{Level set of $V_1, V_2$.}
% \label{fig:1}
% \end{figure}

==> Text/robotic_review.tex <==
possible applications are : welding , writing , sealing/gluing , icing of cake , cleaning , polishing (industry + home applications) ...

X-joint welding ... 
space related tasks: repairing, changing battery, .... 


